A Theory of Sub-Barcodes

From the work of Bauer and Lesnick, it is known that there is no functor from the category of pointwise finite-dimensional persistence modules to the category of barcodes and overlap matchings. In this work, we introduce sub-barcodes and show that there is a functor from the category of factorizations of persistence module homomorphisms to a poset of barcodes ordered by the sub-barcode relation. Sub-barcodes and factorizations provide a looser alternative to bottleneck matchings and interleavings that can give strong guarantees in a number of settings that arise naturally in topological data analysis. The main use of sub-barcodes is to make strong claims about an unknown barcode in the absence of an interleaving. For example, given only upper and lower bounds $g\geq f\geq \ell$ of an unknown real-valued function $f$, a sub-barcode associated with $f$ can be constructed from $\ell$ and $g$ alone. We propose a theory of sub-barcodes and observe that the subobjects in the category of functors from intervals to matchings naturally correspond to sub-barcodes.

==> tikz/colors.tex <==
% !TeX root = ../../main.tex

\def\ca{myred}
\def\cb{myblue}
\def\cc{mygreen}
\def\bgc{gray!20}


==> tikz/diagrams/bar_subcategories.tex <==
% !TeX root=../../main.tex
\begin{center}
\begin{tikzpicture}[very thick,scale=0.75]
\def\l{1.5}
\def\m{5}
\def\h{8.5}
\def\t{7}
\def\u{3}
\def\s{0.3}
\def\n{0.8}
\def\b{1.2}
% AXES
  \draw[semithick,gray]
    (\l-\b-\b,\m) -- (\l-\b-\s,\m)
    (\l+\b+\s,\m) -- (\h-\b-\s,\m)
    (\h+\b+\s,\m) -- (\h+\b+\b,\m)
    (\m,\u-\b-\n) -- (\m,\u-\n-0.2)
    (\m,\u+\n-0.2) -- (\m,\t-\n-0.2)
    (\m, \t+\n-0.2)-- (\m,\t+\b+\n);
% OUTER RECTANGLE
  \draw[semithick,gray] (\l-\b-\b,\u-\b-\n) rectangle (\h+\b+\b,\t+\b+\n);
% SUBBAR
  \draw (\l,\t+\n) node[above] {$\SubBar[P]$};
  \draw[gray,dashed,thin] (\l-\n,\t+\s) -- (\l-\n,\t-\s) (\l+\n,\t+\s) -- (\l+\n,\t-\s);
  \draw (\l-\b,\t-\s) -- (\l+\b,\t-\s) (\l-\n,\t+\s) -- (\l+\n,\t+\s);
%
  \draw (\l-0.5*\s,\m-\s) node[below] {\scriptsize\textit{(coincide above)}};
  \draw[gray,dashed,thin] (\l-\n,\m+\s) -- (\l-\n,\m-\s) (\l+\n,\m+\s) -- (\l+\n,\m-\s);
  \draw (\l-\b,\m-\s) -- (\l+\n,\m-\s) (\l-\n,\m+\s) -- (\l+\n,\m+\s);
% BARC
  \draw (\l,\u-\n) node[below] {$\Barc[P]$};
  \draw[gray,dashed,thin] (\l-\n,\u+\s) -- (\l-\n,\u-\s) (\l+\n,\u+\s) -- (\l+\n,\u-\s);
  \draw (\l-\b,\u-\s) -- (\l+\n,\u-\s) (\l-\n,\u+\s) -- (\l+\b,\u+\s);
%
  \draw (\h-0.5*\s,\m-\s) node[below] {\scriptsize\textit{(coincide above)}};
  \draw[gray,dashed,thin] (\m-\n,\u+\s) -- (\m-\n,\u-\s) (\m+\n,\u+\s) -- (\m+\n,\u-\s);
  \draw (\m-\n,\u-\s) -- (\m+\n,\u-\s) (\m-\n,\u+\s) -- (\m+\b,\u+\s);
% SUBBARop
  \draw (\h,\u-\n) node[below] {$\op{\SubBar[P]}$};
  \draw[gray,dashed,thin] (\h-\n,\u+\s) -- (\h-\n,\u-\s) (\h+\n,\u+\s) -- (\h+\n,\u-\s);
  \draw (\h-\n,\u-\s) -- (\h+\n,\u-\s) (\h-\b,\u+\s) -- (\h+\b,\u+\s);
%
  \draw (\m+0.5*\s,\u-\s) node[below] {\scriptsize\textit{(coincide below)}};
  \draw[gray,dashed,thin] (\h-\n,\m+\s) -- (\h-\n,\m-\s) (\h+\n,\m+\s) -- (\h+\n,\m-\s);
  \draw (\h-\n,\m-\s) -- (\h+\n,\m-\s) (\h-\b,\m+\s) -- (\h+\n,\m+\s);
% BARCop
  \draw (\h,\t+\n) node[above] {$\op{\Barc[P]}$};
  \draw[gray,dashed,thin] (\h-\n,\t+\s) -- (\h-\n,\t-\s) (\h+\n,\t+\s) -- (\h+\n,\t-\s);
  \draw (\h-\n,\t-\s) -- (\h+\b,\t-\s) (\h-\b,\t+\s) -- (\h+\n,\t+\s);
%
  \draw (\m+0.5*\s,\t-\s) node[below] {\scriptsize\textit{(coincide below)}};
  \draw[gray,dashed,thin] (\m-\n,\t+\s) -- (\m-\n,\t-\s) (\m+\n,\t+\s) -- (\m+\n,\t-\s);
  \draw (\m-\n,\t-\s) -- (\m+\b,\t-\s) (\m-\n,\t+\s) -- (\m+\n,\t+\s);

\end{tikzpicture}
\end{center}


==> tikz/diagrams/barcode_equalizer.tex <==
% !TeX root = ../main.tex
\begin{equation}
  \begin{tikzcd}
    \ker(\B,\delta)
        \arrow[r,hook,"k"]
    & \Rep_\B\times\I_\Q
        \arrow[r, shift left=0.7ex, "\B"]
        \arrow[r, shift right=0.7ex, "\delta"']
        \arrow[d, "\pi_2"]
    & \I_\P \\
    %
    \Rep_\B^\delta
        \arrow[u,"\sim" description]
        \arrow[r,"\B^\delta"]
    & \I_\Q &
  \end{tikzcd}
\end{equation}


==> tikz/diagrams/barcode_pullback.tex <==
% !TeX root = ../main.tex
\begin{equation}
  \begin{tikzcd}
    \Rep_\B^\delta
        \arrow[dr,"\sim" description]
        \arrow[drrr, bend left=20,"\B^\delta" description]
        \arrow[dddr, bend right=20,"\rho_\B^\delta" description]
    & & &\\
    %
    & \ker(\B,\delta)
        \arrow[rr,"\rho_1"]
        \arrow[dd,"\rho_2"]
    & & \I_\Q
        \arrow[dd,"\delta"]
    \\
    %
    & & & \\
    %
    & \Rep_\B
        \arrow[rr,"\B"]
    & & \I_\P
  \end{tikzcd}
\end{equation}


==> tikz/diagrams/epimono_dgm.tex <==
% !TeX root=../../main.tex
\begin{equation}\label{dgm:epimono_dgm}
  \def\outbend{10}
  \begin{tikzcd}[row sep=small]
    & \VV'
        \arrow[rrrr, shift left=1,"F" description, gray, bend left=\outbend]
        \arrow[drr,bend right=5, two heads, gray]
    & & & &
    \WW' \arrow[ddddddr, shift left=1, "\varphi_2" description, gray, bend left=\outbend]
        \arrow[ddd,two heads,bend right=10, gray]
    & \\
    %
    & & & \im F
        \arrow[ddrr,bend left=10,"\varphi_F" description, gray]
        \arrow[urr,hook, bend right=5, gray]
        \arrow[ddr, two heads, bend left=5,"e_{\varphi_F}"']
    & & & \\
    %
    & & & & & & \\
    %
    & \im \varphi_1
        \arrow[r,two heads,gray]
        \arrow[uurr,bend left=10,"F_\varphi" description, gray]
        \arrow[ddrr, two heads, bend right=10, gray]
        \arrow[uuu,bend right=10, hook, gray]
    & \im F_\varphi
        \arrow[rr,"\varphi_*" description]
        \arrow[ddr, two heads, bend right=5,"e_{\varphi_*}"]
        \arrow[uur,hook', bend left=5, "m_{F_\varphi}"']
    & & \im \varphi_F
        \arrow[r,hook,gray]
    & \im \varphi_2
        \arrow[dddr,hook, bend right=10, gray]
    & \\
    %
    & & & & & & \\
    %
    & & & \im G
        \arrow[uurr, bend right=10, hook, gray]
        \arrow[drrr, hook, bend right=5, gray]
        \arrow[uur,hook, bend right=5,"m_{\varphi_*}"]
    & & & \\
    %
    \VV \arrow[uuuuuur,shift left=1,"\varphi_1" description, gray, bend left=\outbend]
        \arrow[rrrrrr, shift right=2,"G" description, gray, bend right=\outbend]
        \arrow[urrr,two heads, bend right=5, gray]
        \arrow[uuur,two heads,bend right=10, gray]
    & & & & & & \WW
  \end{tikzcd}
\end{equation}


==> tikz/diagrams/induced_epi.tex <==
% !TeX root = ../../main.tex
\begin{equation}
  \begin{tikzcd}
    & & & \B_{\im F}
        \narrow[dr,two heads,bend left=20,"\cQ_{F\mid_{\im\varphi_1}}"]
        \narrow[dd,two heads,"{\E_{\varphi}}"']
    & \\
    %
    & & & & \B_{\im\varphi_2 F}
        \narrow[dl,two heads,bend left=20,"\rev{\J}_{\varphi_*}"]
    \\
    %
    & & & \B_{\im G}.
    &
  \end{tikzcd}
\end{equation}

% \begin{equation}
%   \begin{tikzcd}
%     & & & \bar_{\im F}
%         \arrow[dr,two heads,bend left=20,"\QQQ_{F\mid_{\im\Phi}}"]
%         \arrow[dd,two heads,"{\RRR_{(\Phi,\Psi)}}"']
%     & \\
%     %
%     & & & & \bar_{\im\Psi F}
%         \arrow[dl,two heads,bend left=20,"\rev{\JJJ}_{\Psi\mid_{\im F}}"]
%     \\
%     %
%     & & & \bar_{\im G}.
%     &
%   \end{tikzcd}
% \end{equation}


==> tikz/diagrams/induced_mono.tex <==
% !TeX root = ../../main.tex
\begin{equation}
  \begin{tikzcd}
    & \B_{\im F}
    & & & \\
    %
    \B_{\im F\varphi_1}
        \narrow[ur,hook',bend left=20,"\J_{F\mid_{\im\varphi_1}}"]
    & & & & \\
    %
    &\B_{\im G}.
        \narrow[ul,hook',bend left=20,"\rev{\cQ}_{\varphi_*}"]
        \narrow[uu,hook,"\ {\M_{\varphi}}"']
    & & &
  \end{tikzcd}
\end{equation}

% \begin{equation}
%   \begin{tikzcd}
%     & \bar_{\im F}
%     & & & \\
%     %
%     \bar_{\im F\Phi}
%         \arrow[ur,hook',bend left=20,"\JJJ_{F\mid_{\im\Phi}}"]
%     & & & & \\
%     %
%     &\bar_{\im G}.
%         \arrow[ul,hook',bend left=20,"\rev{\QQQ}_{\Psi\mid_{\im F}}"]
%         \arrow[uu,hook,"\ {\SSS_{(\Phi,\Psi)}}"']
%     & & &
%   \end{tikzcd}
% \end{equation}


==> tikz/diagrams/induced_mono_epi.tex <==
% !TeX root = ../../main.tex
\begin{equation}
  \begin{tikzcd}
    & \B_{F}
    & \B_{F}
        \narrow[dr,two heads,bend left=20,"\cQ_{F_\varphi}"]
        \narrow[dd,two heads,"{\E_{\varphi}}\, "']
    & \\
    %
    \B_{F_\varphi}
        \narrow[ur,hook',bend left=20,"\J_{F_\varphi}"]
    & & & \B_{\varphi_F}
        \narrow[dl,two heads,bend left=20,"\rev{\J}_{\varphi_*}"]
    \\
    %
    & \B_{G}.
        \narrow[ul,hook',bend left=20,"\rev{\cQ}_{\varphi_*}"]
        \narrow[uu,hook,"\ {\M_{\varphi}}"']
    & \B_{G}.
    &
  \end{tikzcd}
\end{equation}


==> tikz/diagrams/interleaving1.tex <==
% !TeX root = ../main.tex

\begin{minipage}{0.48\linewidth}
  \begin{equation}\label{dgm:old_old_left_interleave}
    \begin{tikzcd}
      \VV(-\epsilon)
        \arrow[rr]
        \arrow[dr] & &
      \VV(\epsilon)\\
      %
      & \UU
        \arrow[ur] &
    \end{tikzcd}
  \end{equation}
\end{minipage}
\begin{minipage}{0.48\linewidth}
  \begin{equation}\label{dgm:old_old_right_interleave}
    \begin{tikzcd}
      & \VV
        \arrow[dr] & \\
      %
      \UU(-\epsilon)
        \arrow[rr]
        \arrow[ur] & &
      \UU(\epsilon)
    \end{tikzcd}
  \end{equation}
\end{minipage}


==> tikz/diagrams/interleaving2.tex <==
% !TeX root = ../../main.tex

\begin{minipage}{0.48\linewidth}
  \begin{equation}\label{dgm:old_left_interleave}
    \begin{tikzcd}[column sep=small]
      \VV(t-\epsilon)
        \arrow[rr,"(\VV\delta)_t"]
        \arrow[dr,"\Phi_t"'] & &
      \VV(t+\epsilon)\\
      %
      & \UU(t)
        \arrow[ur,"\Psi_t"'] &
    \end{tikzcd}
  \end{equation}
\end{minipage}
\begin{minipage}{0.48\linewidth}
  \begin{equation}\label{dgm:old_right_interleave}
    \begin{tikzcd}[column sep=small]
      & \VV(t)
        \arrow[dr,"\Phi_{t+\epsilon}"] & \\
      %
      \UU(t-\epsilon)
        \arrow[rr,"(\UU\delta)_t"']
        \arrow[ur,"\Psi_{t-\epsilon}"] & &
      \UU(t+\epsilon)
    \end{tikzcd}
  \end{equation}
\end{minipage}


==> tikz/diagrams/interleaving3.tex <==
% !TeX root = ../main.tex

\begin{minipage}{0.48\linewidth}
  \begin{equation}\label{dgm:new_left_interleave}
    \begin{tikzcd}
      \VV\e_1
        \arrow[rr,"\VV\delta"]
        \arrow[dr,"\varphi_1"'] & &
      \VV\e_2\\
      %
      & \UU
        \arrow[ur,"\varphi_2"'] &
    \end{tikzcd}
  \end{equation}
\end{minipage}
\begin{minipage}{0.48\linewidth}
  \begin{equation}\label{dgm:new_right_interleave}
    \begin{tikzcd}
      & \VV
        \arrow[dr,"\varphi_1\delta_2"] & \\
      %
      \UU\e_1
        \arrow[rr,"\UU\delta"']
        \arrow[ur,"\varphi_2\delta_1"] & &
      \UU\e_2
    \end{tikzcd}
  \end{equation}
\end{minipage}


==> tikz/diagrams/interleaving_diagrams.tex <==

Given $\\dashv \delta$, $\VV\in\Vec[P]$, $\UU\in\Vec[Q]$ and a factorization $\varphi : \VV\delta\factors \id_\UU$, let $\varphi^\gamma : \UU\gamma_1\Rightarrow \UU\gamma_2$ be defined as the composition
\[\varphi^\gamma \defined \varphi_1\gamma\bdot\eta_1\bdot \eta_2\bdot\varphi_2\gamma_1.\]
visualized
\begin{equation}
  \tikzwrap{
    \natt{\P}{\Q}{\gamma_1}{\gamma_2}{\gamma}
    \nattwo{\Vec}{\UU}{\VV\delta_2}{\varphi_2}}
  \yields
  \anatt{\P}{\Vec}{\UU\gamma_1}{\VV\delta_2\gamma_2}{\varphi_2\gamma}
\end{equation}
\begin{equation}
  \tikzwrap{\natthree{\P}{\Vec}{\UU\gamma_1}{\VV\delta_2\gamma_2}{\VV}{\varphi_2\gamma}{\eta_2}[0.48][0.48]}
  \yields
  \anattdesc{\P}{\Vec}{\UU\gamma_1}{\VV}{\varphi_2\gamma\bdot\eta_2}
\end{equation}

\begin{equation}
  \tikzwrap{
    \natt{\P}{\Q}{\gamma_1}{\gamma_2}{\gamma}
    \nattwo{\Vec}{\VV\delta_1}{\UU}{\varphi_1}}
  \yields
  \anatt{\P}{\Vec}{\VV\delta_1\gamma_1}{\UU\gamma_2}{\varphi_1\gamma}
\end{equation}
\begin{equation}
  \tikzwrap{\natthree{\P}{\Vec}{\VV}{\VV\delta_1\gamma_1}{\UU\gamma_2}{\eta_1}{\varphi_1\gamma}[0.48][0.48]}
  \yields
  \anattdesc{\P}{\Vec}{\VV}{\UU\gamma_2}{\eta_1\bdot\varphi_1\gamma}
\end{equation}

\begin{equation}
  \tikzwrap{\natthree{\P}{\Vec}{\UU\gamma_1}{\VV}{\UU\gamma_2}{\varphi_2\gamma\bdot\eta_2}{\eta_1\bdot\varphi_1\gamma}[0.48][0.48]}
  \yields
  \anattdesc{\P}{\Vec}{\UU\gamma_1}{\UU\gamma_2}{\varphi^\gamma}
\end{equation}

Regarding $\id_\VV$ and $\varphi^\gamma$ as functors $\F{\P}\to \F{\Vec}$, let $\varphi^\gamma_* : \id_\VV\Rightarrow \varphi^\gamma$ denote the natural transformation visualized
\begin{equation}
  \anatt{\F{\P}}{\F{\Vec}}{\id_\VV}{\varphi^\gamma}{\varphi^\gamma_*}
\end{equation}


==> tikz/diagrams/matching_pullbacks.tex <==
% !TeX root = ../main.tex

\begin{equation}
  \begin{tikzcd}
    \Rep_\B^\delta
        \narrow[dddr,bend right=20]
        \arrow[drrr, bend left=20,"\B^\delta"]
        \narrow[dr, hook, "M^{\delta\times\id}"]
    & & & & & \Rep_\Ar^\gamma
        \narrow[dddr,bend right=20]
        \arrow[drrr, bend left=20,"\Ar^\gamma"]
    & & & \\
    %
    & \Rep_\Ar
        \arrow[rr,"\Ar"]
        \arrow[dd,"M"]
    & & \I_\Q
      \arrow[dd,"\delta"]
    & & & \Rep_\B
      \arrow[rr,"\B"]
      \narrow[ul,two heads,"M^{\id\times\delta}"']
    & & \I_\P
      \arrow[dd,"\gamma"]
    \\
    %
    & & & & & & & &\\
    & \Rep_\B
      \arrow[rr,"\B"]
    & & \I_\P
    & & & \Rep_\Ar
      \arrow[rr,"\Ar"]
      \narrow[uu,"M"]
    & & \I_\Q
  \end{tikzcd}
\end{equation}


==> tikz/diagrams/slices.tex <==
% !TeX root=../../main.tex
% \begin{equation}
%   \begin{tikzcd}[column sep=tiny,row sep=large]
%     && & (\cat{C}\downarrow b) & && & (b\downarrow\cat{C}) &
%     \\
%     %
%     && & a \arrow[d, "f"] &
%     && & &
%     \\
%     %
%     (objects) && & b &
%     &&
%     & b \arrow[d, "g"]
%     & \\
%     %
%     && && &&
%     & c &
%     \\
%     %
%     && a'\arrow[rr,"v"]
%         \arrow[dr,"f'"']
%     && a
%     && & &
%     \\
%     %
%     (arrows)
%     &&
%     & b \arrow[ur,"f"']
%     & &&
%     & b \arrow[dr,"g'"] &
%     \\
%     %
%     && &&
%     && c\arrow[ur,"g"]
%         \arrow[rr,"u"]
%     && c'
%   \end{tikzcd}
% \end{equation}

% \begin{equation}
%   \begin{tikzcd}[sep=tiny]
%     && a\arrow[dd,"f"'] && && a'\arrow[rr,"v"]\arrow[ddr,"f'"'] && a\arrow[ddl,"f"]\\
%     (objects) && && (arrows) &&&&\\
%     && b && &&& b  &
%   \end{tikzcd}
% \end{equation}
% \begin{equation}
%   \begin{tikzcd}[sep=tiny]
%     && b\arrow[dd,"g"'] && &&& b\arrow[ddl,"g"']\arrow[ddr,"g'"] &\\
%     (objects) && && (arrows) &&&&\\
%     && c && && c\arrow[rr,"u"]  && c'
%   \end{tikzcd}
% \end{equation}


==> tikz/intervals/coincides_above.tex <==
% !TeX root = ../main.tex

\[
    \begin{tikzpicture}[very thick]
        %COINCIDES ABOVE
      \draw (0.5,0) node {\dots} (1,0) -- (3,0) (3.5,0) node {$J$};
      \draw (0.5,0.45) node {\dots} (1,0.45) -- (3,0.45) (3.5,0.45) node {$I$};

        %COMMENT OUT TO REMOVE ENDPOINT DOTS
      \foreach \p in {(3,0), (3,0.45)}
          \filldraw \p circle (0.05);

    \end{tikzpicture}
\]


==> tikz/intervals/survive.tex <==
% !TeX root = ../main.tex
\[
    \begin{tikzpicture}[very thick]
        \draw (2.5,0) -- (4.5,0);
        \draw (2,0) node {$\dots$};
        \draw (5,0) node {$\dots$};
        \filldraw (2.5,0) circle (0.05) node[below,black,yshift=-3] {$b$};
        \filldraw (4.5,0) circle (0.05) node[below,black,yshift=-6] {$c$};
    \end{tikzpicture}
\]


==> tikz/matching/matching.tex <==
% !TeX root = ../main.tex
%\[
\begin{center}
\scalebox{0.6}{
    \begin{tikzpicture}[very thick,fill=black]
        \draw (0,0) ellipse (0.5 and 2);
        \draw (3,0) ellipse (0.5 and 2);

        \foreach \p in {(0,0.5),(0,-0.5),(0,1),(0,-1),(0,0),(3,0),(3,-1),(3,1)}
            \filldraw \p circle (0.075);

        \draw[->,shorten >=5pt] (0,0.5) -- (3,-1);
        \draw[->,shorten >=5pt] (0,-1) -- (3,0);
        \draw[->,shorten >=5pt] (0,1) -- (3,1);
    \end{tikzpicture}
}
\end{center}
%\]


==> tikz/matching/matching_composition.tex <==
% !TeX root = ../main.tex
%\[
\begin{center}
\scalebox{0.6}{
    \begin{tikzpicture}[very thick,fill=black]
        \draw (0,0) ellipse (0.5 and 2);
        \draw (3,0) ellipse (0.5 and 2);
        \draw (6,0) ellipse (0.5 and 2);

        \foreach \p in {(0,0.5),(0,-0.5),(0,1),(0,-1),(0,0),(3,0),(3,-1),(3,1),(6,0),(6,-1.5),(6,1.5),(6,0.7),(6,-0.7)}
            \filldraw \p circle (0.075);

        \draw[->,shorten >=5pt] (0,0.5) -- (3,-1) -- (6,-0.7);
        \draw[->,shorten >=5pt] (0,-1) -- (3,0) -- (6,1.5);
        \draw[->,shorten >=5pt] (0,1) -- (3,1) -- (6,0.7);
    \end{tikzpicture}
}
\end{center}
%\]


==> tikz/matching/matching_reverse.tex <==
% !TeX root = ../../main.tex
%\[
\begin{center}
\scalebox{0.6}{
    \begin{tikzpicture}[very thick,fill=black]
        \draw (0,0) ellipse (0.5 and 2);
        \draw (3,0) ellipse (0.5 and 2);

        \foreach \p in {(0,0.5),(0,-0.5),(0,1),(0,-1),(0,0),(3,0),(3,-1),(3,1)}
            \filldraw \p circle (0.075);

        \draw[<-,shorten >=5pt] (0,0.5) -- (3,-1);
        \draw[<-,shorten >=5pt] (0,-1) -- (3,0);
        \draw[<-,shorten >=5pt] (0,1) -- (3,1);
    \end{tikzpicture}
}
\end{center}
%\]


==> tikz/tda/approx.tex <==
% !TeX root = ../../main.tex

\begin{center}
\begin{tikzpicture}[thick]
    % X-COORDINATE STRETCH
    \def\k{1.7};
    % EPSILON
    \def\e{0.7};


    \draw[mygreen, very thick] plot coordinates{ (\k*0,1+\e) (\k*1,2+\e) (\k*2,1.5+\e) (\k*3,3+\e) (\k*4,2+\e) (\k*5,4+\e)};
    \draw[myblue, very thick] plot coordinates{ (\k*0,1-\e) (\k*1,2-\e) (\k*2,1.5-\e) (\k*3,3-\e) (\k*4,2-\e) (\k*5,4-\e)};

    \foreach \x/\y/\f in { 0/1/0.2, 1/2/0.3, 2/1.5/0.5, 3/3/0.7, 4/2/0.2, 5/4/0.3} {
      \draw[|-|, semithick] (\k*\x,\y+\f) -- (\k*\x,\y-\f);
    }
    % THE FUNCTION
    \draw[dashed] plot coordinates{ (\k*0,1) (\k*1,2) (\k*2,1.5) (\k*3,3) (\k*4,2) (\k*5,4)};
    \draw[myred, very thick] plot[smooth,tension=1] coordinates{ (\k*0,1) (\k*1,2) (\k*2,1.5) (\k*3,3) (\k*4,2) (\k*5,4)};
    % POINTS
    \foreach \p in {(\k*0,1), (\k*1,2), (\k*2,1.5), (\k*3,3), (\k*4,2), (\k*5,4)} { \filldraw[myred] \p circle (0.05);}
    % LABELS
    \draw (\k*5,4+\e) node[mygreen, very thick, right] {\Large$g$};
    \draw (\k*5,4) node[right, very thick, right] {\Large$f$};
    \draw (\k*5,4-\e) node[myblue, very thick, right] {\Large$l$};

    DRAW EPSILON
    \draw[|-|, semithick] (\k*5+1,4+\e) edge node[right, thick] {$2\varepsilon_{\max}$} (\k*5+1,4-\e);
\end{tikzpicture}
\end{center}


==> tikz/tda/haunting_curves.tex <==
\begin{center}
\begin{tikzpicture}[very thick]
%%% Curves
  \draw[red] plot [smooth] coordinates {(0,2) (1,-2) (2,2) (3,-2) (4,2) (5,-2) (6,3) (7,3) (8,3)} node[right] {$f$};
  \draw[black,yshift=-20] plot [smooth] coordinates {(0,2) (1,-2) (2,-2) (3,-2) (4,2) (5,-2) (6,3) (7,3) (8,3)} node[right] {$g$};
  \draw[blue,yshift=-40] plot [smooth] coordinates {(0,2) (1,-2) (2,-2) (3,-2) (4,2) (5,-2) (6,2) (7,-2) (7.5,3)};
  \draw[blue,yshift=-40] (7.5,3)-- (8,3) node[right] {$h$};

%%% Barcodes
%    \draw[red]  (-4,-1) --   (-4, 1)
%                (-4.2,-1) -- (-4.2,1)
%                (-4.4,-1) -- (-4.4,1)
%                (-4.6,-1) -- (-4.6, 2.2)
%                (-4.8,2) --  (-4.8,2.2);

    \draw[black,yshift=-20]
                (-1.4,-2.25) -- (-1.4,2)
                (-1.6,-2.25) -- (-1.6,2)
                (-1.2,-2.25) -- (-1.2, 3.4)
                (-1.8,-2.25) -- (-1.8,-2);
%                (-1,3) --  (-1,3.4);

%    \draw[blue,yshift=-40]
%                (-3.2,-1) -- (-3.2, 1)
%                (-3.4,-1) -- (-3.4,1)
%                (-3.6,-1) -- (-3.6,1)
%                (-3.8,-1) -- (-3.8, 2.2)
%                (-4,-1)   -- (-4,-0.8);

%    \draw[purple]
%                (9,-2.4) -- (9,2.3)
%                (9.2,-2.4) -- (9.2,1.2)
%                (9.4,-2.4) -- (9.4,1.2)
%                (9.6,-2.4) -- (9.6,1.2);

    \draw
                (-3.6,-2) -- (-3.6,0.6)
                (-3.4,-2) -- (-3.4,0.6)
                (-3.2,-2) -- (-3.2,1.6);

%    \draw[yshift=-20] (1.3,-2.25) circle (0.1);
%    \draw[yshift=-20] (1.3,-2.3) circle (0.1);

    \draw (-2.5,0) node {$\sqsubseteq$};
    \draw (-3.5,3) node {\tiny$\Bar(\H\Sub(f\ge h))$};
    \draw (-1.25,3) node {\tiny$\Bar(\H\Sub(g))$};
\end{tikzpicture}
\end{center}

